Visual Question Answering: which investigated applications?

Visual Question Answering (VQA) is an extremely stimulating and challenging research area where Computer Vision (CV) and Natural Language Processig (NLP) have recently met. In image captioning and video summarization, the semantic information is completely contained in still images or video dynamics, and it has only to be mined and expressed in a human-consistent way. Differently from this, in VQA semantic information in the same media must be compared with the semantics implied by a question expressed in natural language, doubling the artificial intelligence-related effort. Some recent surveys about VQA approaches have focused on methods underlying either the image-related processing or the verbal-related one, or on the way to consistently fuse the conveyed information. Possible applications are only suggested, and, in fact, most cited works rely on general-purpose datasets that are used to assess the building blocks of a VQA system. This paper rather considers the proposals that focus on real-world applications, possibly using as benchmarks suitable data bound to the application domain. The paper also reports about some recent challenges in VQA research.

==> reviews.tex <==
\section*{REBUTTAL}
Dear Editor,\\
First of all, we would like to thank once again the reviewers for their constructive remarks. We completed the requested revision of our manuscript \textit{Visual Question Answering: which investigated applications?} submitted to Pattern Recognition Letters on the basis of the observations made by the reviewers and the editor.
In the following, you will find the details of each of them. Reviewer questions have been coloured in blue whereas our responses have been coloured in red.
Thanks again for all your feedback that led us to largely improve the paper.\\ 

\noindent
Best Regards, \\Authors

\textcolor{blue}{Reviewer #1} 
In this paper, the authors survey Visual Question Answering proposals. In doing this, the authors focused on real-world applications together with the exploited datasets.

The paper is well-written and well-structured. The "Introduction" section is very readable; aims and scope of the paper are clearly exposed and reported. The authors propose an interesting taxonomy (i.e., the rest of the paper) for the VQA proposals, in which can be seen a careful analysis of the current state-of-the-art. Reading the paper, the taxonomy and, in particular, Table 2, the reader can be focused on a novel interpretation of this topic, in which challenging techniques for specific domains as well as emerging challenges are well pointed out. This Reviewer has not observed typos or oversights, also the overall style seems to be appropriate.

\textcolor{red}{Authors} We thank the reviewer for the positive comment to our work; the taxonomy indeed has been object of very deep reasoning, in order to let the reader to understand our point of view of the topic. 

\textcolor{blue}{Reviewer #2} 
The paper presents a survey of VQA (Visual Question Answering) research. Different from some recent surveys, the authors argue that summarization in this paper is done by application domains (which is lacking in other surveys),  rather than by methodologies or algorithms. For such purpose, the different sections of the paper are devoted to different application domains, e.g. for medical purposes, for aiding visually impaired people, for education/culture, for advertising, etc.
\textcolor{red}{Authors} We thank the reviewer for the precise analysis of our work. We noticed that the none amongst the surveys analysed has focused on the application domain, rather they faced the description of the methods, going more or less in the deep with the explanation. From our point of view, the application domain, which is quite never discussed, has the same importance.

\textcolor{blue}{R2}
In its current form, the paper mainly consists of plain text (plus two tables) "travelling" through the different relevant references of each domain, with a mention to the data employed and a high level indication of the algorithms employed. While this must be a part of a review paper, this reviewer is missing some other "summarization" elements that would be useful in a review paper to help the reader to get an overall view without having to dive into the complete text. For example:

-A graphic/picture showing the "image featurization-text featurization-joint comprehension-answer" concept. In other words, what are the main steps of a VQA system

-A list of the most recurrent features/algorithms employed in the literature for each sub-task, e.g. in a table

-Images of each application domain showing actual examples of images+questions

Another important aspect that I am missing is a mention to the performance metrics usually employed, together with accuracy numbers of the referenced works (or at least the best performing ones). In the present version, the reader cannot get an idea of "how good" is the state of the art in the topic, this has to be looked at elsewhere in the references (or another surveys). Some works make use of the same database (in the context of competition benchmarks), so giving numbers would also be of help comparatively.

\textcolor{red}{Authors} We definitely agree with the reviewer and we had the same plan for the paper at the beginning. We did not insert these information in the submitted version given the limited space at our disposal. However, given the possibility to use an extra page for answering the suggestions of the reviewer, we inserted in the paper all the required information. In particular, at page 2 and page three you can find the images of the typical VQA approach and of the specific applications. Moreover, Table one has been enhanced with two more columns, related to the approach used and to the best results obtained, when compared on the same dataset.


\textcolor{blue}{R2}
Other minor questions:

Section 2 is quite long, you may want to consider dividing the text in a few paragraphs.

Page 4, first paragraph: "In Bansal et al., the proposed med-VQA..." -> the reference is missing the year, it seems that the compiler is not catching it properly.

Section 6: VQA and advertising. It is mentioned that the aims may include understanding which part of an ad impresses users the most, or which part is more attractive. Does this imply that the reaction of the user to the ad is also captured? If not, how the mentioned aims are achieved?

\textcolor{red}{Authors}
We are grateful to the reviewer for giving us the opportunity to improve the work. Actually, both of the possibilities are available. However, in one of the papers described (Hussain et al. (2017)) this is clearly explained. There are several ways to proceed: as an example technique for detecting what is surprising or funny in an ad can be used, or methods for detecting symbolisms in the ads. This can be done by using an attention model. The model should be difffentiated according to the aim of the ad (e.g. funny ads need different attention models with respect to other types of ads).


==> sections/oldtable.tex <==


\begin{table*}[]
\centering
%\scriptsize
\footnotesize
\label{t:final}
\caption{A summary of application domains tackled by VQA literature with a summary of the features of the datasets used as benchmarks.}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Domain} & \textbf{Reference(s)} & \textbf{Dataset} & \textbf{Dataset Size} & \textbf{Notes on Dataset} \\ 
    \hline
    Medical & \cite{vu2020question}, \cite{ren2020cgmvqa}, \cite{allaouzi2019encoder}  & ImageCLEF 2019 & 3200 images & 12,792 Q\&A \\ 
      & \cite{bansalmedical}, \cite{al2019just}, \cite{bghiel2019visual} &   &   & \\
      & \cite{lubna2019mobvqa}, \cite{nguyen2019overcoming}, \cite{vu2019ensemble}  &  &  &  \\
      & \cite{yan2019zhejiang}, \cite{shi2019deep}, \cite{kornuta2019leveraging} &  &   &  \\
      & & & &\\
      & \cite{zhou2018employing}, \cite{allaouzi2018deep} & ImageCLEF 2018 & 2866 images & 6,413 Q\&A \\
      & \cite{ambati2018sequence}, \cite{abacha2018nlm} &  &  &  \\
      & \cite{peng2018umass}, \cite{liu2019effective} &  &  &  \\
       \hline
    Visually & \cite{gurari2019vizwiz} & VizWiz-Priv & 5537 images & 1403 Q\&A\\
     impaired& \cite{vizwiz} & VizWiz & 31000 images & 31000 Q \& 10 A each\\
      &\cite{Anderson_2018_CVPR}& VQA v2.0 Dataset & 1.1M images & 1.1M Q\&A\\
     &\cite{weiss2019navigation} & SEVN Simulator & - & - \\
     \hline
    Video & \cite{li2019isee} & RAP & 587 hours of video & 84928 imgs \&72 attrs\\
    Surveillance& \cite{TOOR2019111} & BOAR + BTV & $\sim$45K images, 5 videos & $\sim$23K Q, 101 classes \\
     & \cite{6818956} & Homemade & 2 short videos & 5 captions each\\
     \hline
    Cultural & \cite{Bongini2020VisualQA} & Annotated Artpedia  &  30 images & $\sim$120 Q\&A   \\ 
    Heritage & \cite{Sheng2016ADF} & Homemade & 16 images, 444 texts & 805 Q\&A \\\hline
    Advertising & \cite{Hussain_2017_CVPR} & Homemade  &  64832 images, 3477 videos & $\sim$273000 Q\&A \\ 
     & \cite{park2019ads} & Real-ad: Homemade & 3747 images & 500k impressions \\
     \hline
    Misc & \cite{Chou2020VisualQA}: $360^\circ$ data & Homemade & 1490 images in $360^\circ$ & 16945 Q\&A \\
     & \cite{sampat2020diverse}: image+text inference & Homemade & 10209 images, 9156 texts & 9267 Q\&A \\
     & \cite{wang2020long}:long video & TACoS-QA & 185 long videos & 21310 Q\&A \\
     & \cite{wang2020long}: long video & MSR-VTT-QA & 3852 long videos & 19748 Q\&A \\ 
     & \cite{abdelnour2019visual}: acoustic QA & Homemade & 7500 audio scenes & 300000 Q\&A \\
     & \cite{hosseinabad2020multiple}: multiple answers & Homemade & 85321 images of icons & 429654 Q\&A \\
     & \cite{bhattacharya2019does}: multiple answers & VQA 2.0+VizWIz+labels & 44955 images & 224775 Q\&A \\
     & \cite{toor2019question}: query properties & COCO-A+VG+classes & 19431 images, 342 classes & $\sim$80000 Q\&A \\
     & \cite{teney2019actively}: more questions+external data & VQA-CP v2+COCO & 325721 images & $\sim$1.5M Q \& $\sim$15M\\
     \hline
\end{tabular}
\end{table*}

